A Flexible Adaptive Stable Clustering Algorithm for Archive-Scale Online Mass Spectrometry

Modern online mass spectrometry generates multi-terabyte data streams critical for understanding Earth's environmental systems. However, extracting actionable chemical insights from these repositories is impeded by a computational bottleneck: existing clustering methods force a compromise among scalability, metric flexibility, and algorithmic stability. Here, we introduce Flexible Adaptive Stable Clustering (FASC), a dynamical systems framework that resolves these constraints by architecturally decoupling the similarity kernel from rigorous optimization logic. Unlike legacy heuristics that suffer from stochastic drift and algorithmic blending, FASC employs a Density-Augmented Similarity Selection rule and geometric constraints to guarantee deterministic, order-independent convergence. After validating FASC on canonical machine-learning ground truths (achieving >99.5% cluster purity and 0.99 Adjusted Rand Index), we deployed the framework on 25 million mass spectra of atmospheric aerosols. Demonstrating strictly linear empirical runtime scaling (O(N)), FASC autonomously mapped atmospheric aging pathways of secondary inorganic aerosols while isolating ultra-rare industrial tracers (<0.2% abundance), providing a scalable infrastructure for mining environmental big data.

==> manuscript_subsection_iteration.tex <==
\subsection{Convergence Analysis and Empirical Stability}

We evaluate the inter-iteration behavior of FASC by coupling the deterministic schedule of Algorithm~\ref{alg:fasc} with the Lyapunov-based guarantees derived in \supptextref{supp:text-s5}. Because Phase~1 computes all assignments against a fixed representative set and resolves ties deterministically, any permutation of the input stream follows the same optimisation path once the seed is fixed, satisfying the stability definition from \supptextref{supp:text-s4}. 
Formally, Lemmas~\ref{lem:assignment}--\ref{lem:centroid} prove that the assignment and centroid update phases strictly improve the Bregman objective $\mathcal{L}_\phi$ (under SF) or the potential $\Psi$ (under DASS). 
In practical terms, this drives the system toward a geometrically stable configuration where no single sample reassignment or representative shift can further improve the clustering quality.

To maximize adaptability and throughput, FASC performs structural edits (merges and promotions) immediately upon threshold satisfaction. 
While this aggressive strategy prioritizes efficient capacity adjustment over strict step-wise monotonicity, the integrated limit-cycle safeguard (Theorem~\ref{thm:cycle}) guarantees deterministic termination. 
By monitoring the hashed state history, Phase~3 automatically detects if these edits induce an oscillation and recovers the optimal state, acting as a rigorous theoretical safety net.
Although the DASS potential theoretically admits a vast number of strict gains, empirical trajectories are highly efficient.
In the 24~million-spectrum experiment described in Methods, the convergence monitors fall below the strict tolerance of $10^{-3}$ well before twenty sweeps.

\suppfigref{fig:si_iter_similarity} illustrates this rapid stabilization for the dual-cosine kernel ($\tau_{\text{intra}}=\tau_{\text{inter}}=0.7$, $K_{\max}=50$). 
The inter-iteration similarity dips to $\approx 0.986$ only during the initial phase of rapid cluster discovery but rebounds above $0.999$ by the tenth pass.
Crucially, the active-cluster trace saturates at $K_{\max}$ within $\sim 20$ passes, implying that FASC rapidly identifies the chemical diversity of the aerosol population without generating spurious, transient clusters.
Simultaneously, the provisional outlier pool shrinks by over $80\%$ within sixty passes (\suppfigref{fig:si_outliers}), leaving only chemically unique spectra. 
To date, no large-scale run has triggered the limit-cycle guard, confirming that the algorithm’s dynamics align naturally with the underlying structure of mass spectrometric big data.

